Privacy and Truthful Equilibrium Selection for Aggregative Games

We study a very general class of games --- multi-dimensional aggregative games --- which in particular generalize both anonymous games and weighted congestion games. For any such game that is also large, we solve the equilibrium selection problem in a strong sense. In particular, we give an efficient weak mediator: a mechanism which has only the power to listen to reported types and provide non-binding suggested actions, such that (a) it is an asymptotic Nash equilibrium for every player to truthfully report their type to the mediator, and then follow its suggested action; and (b) that when players do so, they end up coordinating on a particular asymptotic pure strategy Nash equilibrium of the induced complete information game. In fact, truthful reporting is an ex-post Nash equilibrium of the mediated game, so our solution applies even in settings of incomplete information, and even when player types are arbitrary or worst-case (i.e. not drawn from a common prior). We achieve this by giving an efficient differentially private algorithm for computing a Nash equilibrium in such games. The rates of convergence to equilibrium in all of our results are inverse polynomial in the number of players $n$. We also apply our main results to a multi-dimensional market game. Our results can be viewed as giving, for a rich class of games, a more robust version of the Revelation Principle, in that we work with weaker informational assumptions (no common prior), yet provide a stronger solution concept (ex-post Nash versus Bayes Nash equilibrium). In comparison to previous work, our main conceptual contribution is showing that weak mediators are a game theoretic object that exist in a wide variety of games -- previously, they were only known to exist in traffic routing games.

==> Extensions.tex <==
\section{Discussion}\label{s.exten}
Can we have a $\poly(1/\alpha, n, m)$ algorithm that computes an
approximate equilibrium for multi-dimensional summarization game?
Currently, we have an algorithm with runtime proportional to
$(1/\alpha)^d$. 


%\sw{Removed the following since we have addressed them in the
%selection section.}

% \subsection{Non-binary discrete valued actions}\label{s.nonbin}

% The algorithms PrivateSummNash and PrivateEquilibriumSelection can
% still work when each player selects an action from an arbitrary
% discrete set, rather than a binary action. For computational
% efficiency, we require an ordering $\succsim$ over the action space
% $A$ of each player as follows. Since we are considering anonymous
% games, all players must have the same action space and the same
% ordering over actions for all players.
% \[ V(a_i, s_{-i}) \leq V(a_i^{\prime}, s_{-i}) \; \Longleftrightarrow
% \; a_i \succsim a_i^{\prime} \] for all $i$ and $a_i, a_i^{\prime} \in
% A$.

% This ordering allows Algorithm 3 to efficiently compute $S_{min}$ and
% $S_{max}$. To compute $S_{min}$ (resp. $S_{max}$), select the action
% profile where each player plays the action from their best response
% set that is lowest (highest) on this ordering. Without such an
% ordering, we may need to check exponentially many strategy profiles,
% which cannot be done efficiently or privately. With the ordering, it
% can be done in two queries for each $\alpha$-interval.
%\sw{this is covered by section 3}


% \subsection{Continuous valued actions}

% It may be the case that each player has a continuum of actions, say
% normalized to $[0,1]$, rather than a binary choice. This would cause
% the summarization function to be continuous valued rather than
% discrete. The algorithms PrivateSummNash and
% PrivateEquilibriumSelection can again be modified to run in this
% setting, under some additional conditions. Instead of defining a set
% of payoff functions $\F^i_b$ for $b \in A$, we instead consider payoff
% functions for each agent that takes two inputs: the player's action
% and the summarization value. Define $\F_i(a, S)$ to be the payoff of
% agent $i$ when she plays action $a \in [0,1]$ and the summarization
% value is $S$.

% The first condition we need is an ordering over actions, as in Section
% \ref{s.nonbin}.
% \[ V(a_i, s_{-i}) \leq V(a_i^{\prime}, s_{-i}) \; \Longleftrightarrow
% \; a_i \succsim a_i^{\prime} \] for all $i$ and $a_i, a_i^{\prime} \in
% A$. As before, this will allow us to efficiently compute $S_{min}$ and
% $S_{max}$ for each $\alpha$-interval.

% Additionally, we require each player's payoff to be Lipschitz
% continuous in the the action played.
% \[ |\F_i(a_1, S) - \F_i(a_2, S)| \leq \delta |a_1 - a_2| \] for all
% $i$, $S$, and $a_1, a_2 \in [0,1]$. This requirement, combined with
% the assumption of bounded derivatives on utility functions, presented
% in Section \ref{s.intro}, gives the following continuity condition on
% payoffs:
% \[ |\F_i(a_1, S_1) - \F_i(a_2, S_2)| \leq \delta |a_1 - a_2| + \rho
% |S_1 - S_2|\]

% We motivate these assumptions with the following negative example.
% When the summarization function is allowed be non-monotone and have
% discontinuities, the set of finite approximations to the best
% equilibrium has measure zero, so we should not hope that our algorithm
% (or any algorithm that runs in finite time) can guarantee a finite
% (expected) approximation ratio to the best equilibrium.
% \begin{example} Graph 2 of notes: $V(S)$ is zero everywhere except at
% a single point $S^*$, where $V(S^*) = S^*$.
% \end{example} The imposed continuity conditions prevent such examples,
% and ensure that the summarization function is well-behaved.
% Intuitively, if the summarization function is badly behaved, we should
% not expect to get back a good approximation.

% Further, we show by the following negative result that
% PrivateEquilibriumSelection as written in Section \ref{s.select} can
% no longer provide good approximation guarantees. We use this negative
% example to motivate modifications to the algorithm.
% \begin{prop} No instantiation of PrivateEquilibriumSelection that runs
% in finite time can guarantee a finite approximation ratio to the best
% equilibrium.
% \end{prop}
% \begin{proof} Graph 1 of notes, $V(S)$ touches the diagonal only at
% zero and at a single point in $(1-\alpha, 1)$. For any $\alpha$ chosen
% as a discretization parameter, such a function exists.
% \end{proof}

% The modification we make to the algorithm is to have players report a
% set of $\delta + \rho \alpha$-approximate best responses, rather than
% their $\rho \alpha$ best responses.

% \begin{theorem} PrivateEquilibriumSelection with $\delta + \rho
% \alpha$-approximate best responses outputs a $\delta + \rho
% \alpha$-approximate Nash equilibrium.
% \end{theorem}







==> PrivateSummNash.tex <==
\section{Private SummNash Algorithm}


In this section, we present a privatized version of the $\SN$
algorithm proposed in \cite{KM02}. Our algorithm is essentially the
same as \SN, except that it only accesses the private data through
\SV. In particular, the algorithm iterates through at most $O(n)$
strategy profiles and halts as soon as it finds an approximate Nash
equilibrium.

% First, the algorithm constructs an $\alpha$-approximate game
% $\hat{\mathcal{G}}$ to the original game $\mathcal{G} = (S,\{(\F_0^i,
% \F_1^i)\}_{i=1}^n$: for each player $i$ and each action $b$, define
% $\hF_b^i(z) = \F_b^i(k\alpha)$ for all $z\in I_k= [k\alpha,
% (k+1)\alpha)$.
%\sw{ this is not necessary. }

For each summarization value $s$, we define the \emph{apparent best
  response} for player $i$ to be $\br_i(s) = \arg\max_{a\in A}
\{\F_a^i(s)\}$, breaking ties arbitrarily. Note that exact \emph{best
  response} is played against the other players' strategies $x_{-i}$
instead of an explicit summarization value $s$, but here we ignore the
effect the player's action has on the summarization value, which is
bounded by $\gamma$ by our assumption (the player is simply reasoning
about the utility of playing action 0 or 1 as if the summarization
value were \emph{promised} to be $s$). Furthermore, we define function
$V(s) = S(\br(s))$, and argue that the approximate fixed point of $V$
gives an approximate Nash equilibrium of the game.


\begin{algorithm}[h!]
 \caption{Private \SN }
 \label{alg:psn}
 \begin{algorithmic}
   \INDSTATE[0]{\textbf{Input}: An $n$-player $(\gamma,
     \rho)$-summarization game $(S, \{(\F_a^i)\})$,
     and a privacy cost $\eps$} \INDSTATE[0]{\textbf{Output:} An $(\xi
     + 2\gamma\rho)$-approximate Nash equilibrium}

    % \INDSTATE[1]{\textbf{for} each player $i$ and action $b\in
    %   A$, construct the $\alpha$-approximate payoff function
    %   $\F^i_b$: for every $\alpha$-interval $I_k = [k\alpha,
    %   (k+1)\alpha)$, $\F(z) = \F_b^i(k\alpha)$ for all $z\in I_k$. }
    \INDSTATE[1]{\textbf{let} $\alpha = \xi / 10\rho$}
    % \INDSTATE[1]{\textbf{for} each $0\leq k \leq 1/\alpha - 1$,
    %   \textbf{let} interval $I_k = [k\alpha, (k+1)\alpha]$  }
    % \INDSTATE[1]{\textbf{let} the mapping $V$ be defined as $V(I_k) = S(\br(I_k))$}
    \INDSTATE[0]{\textbf{Case 1}} \INDSTATE[1]{\textbf{for} each
      $0\leq k \leq 1/\alpha - 1$, define a query $Q_k$ on the
      players' private payoff functions:}
      \[Q_k = | V(k\alpha) -  k\alpha |\]
    \INDSTATE[1]{\textbf{let} $\{a_k\}=\SV(\{\F_a^i\}, \{Q_k\},
      4\alpha, 1, \eps/3 )$}
    \INDSTATE[3]{\textbf{if} we have some  $a_t \neq \perp$  \textbf{then Output}  $\br(t\alpha)$}
    \INDSTATE[0]{\textbf{Case 2}}
    \INDSTATE[1]{\textbf{for} each $1\leq k\leq 1/\alpha - 1$, define query
      $Q'_k$ on the players' private payoff functions:}
      \[ Q'_k = \max\left( \min(0, k\alpha - V((k -1 )\alpha)
, -2\alpha \right) + \max\left( \min\left(0, V(k\alpha) - k\alpha
\right), -3\alpha \right)
      \]
    
    \INDSTATE[1]{\textbf{let} $\{a'_k\}=\SV(\{\F_a^i\}, \{Q'_k\},
     4\alpha , 1, \eps/3 )$}
    \INDSTATE[2]{\textbf{if} all  $a'_k = \perp$  \textbf{then} Abort.}
    \INDSTATE[2]{\textbf{else let } $l$ be the index such that $a'_l
      \neq \perp$}
    \INDSTATE[1]{\textbf{for} each $0\leq j\leq n$, \textbf{let}
      strategy profile $x^j$ be defined as}
    \[
    x^j_i = \begin{cases}
      \br_i(l\alpha) \mbox{ if }i\leq j\\
      \br_i((l-1)\alpha)\mbox{ otherwise}
      \end{cases}
    \]
      \INDSTATE[2]{\textbf{let } query $Q_j'' = S(x^i)$} 
    \INDSTATE[2]{\textbf{let} $\{a''_j\}=\SV(\{\F_a^i\}, \{Q''_i\},
      \gamma/2 + \alpha, 1, \eps/3 )$}
    \INDSTATE[3]{\textbf{if} some $a''_{j'} \neq \perp$  \textbf{then
        Output } $x^{j'}$ \textbf{else } Abort.} 
  \end{algorithmic}
\end{algorithm}


\begin{theorem}\label{thm:psn-privacy}
  \Cref{alg:psn} satisfies $\eps$-joint differential privacy.
\end{theorem}

\begin{proof}
Note that the  \Cref{alg:psn} accesses the data only through \SV,
and thus the strategy profile selection as a public message
satisfies $\eps$-differential privacy by composition theorem. Also,
the action each player is playing is a function of public message and
 her own private payoff functions, so the 
mechanism satisfies $\eps$-joint differential privacy.
\end{proof}

\begin{restatable}{theorem}{psnutility}
%\begin{theorem}
\label{thm:psn-utility}
Suppose $\gamma = 1/n$, then with probability at least $1-\beta$, \Cref{alg:psn} computes
a $O(\gamma\rho + \xi)$-approximate Nash equilibrium as long as
$n \geq \tilde{O}\left(\frac{\rho\log(1/\beta)}{\xi\eps}\right)$.
%\end{theorem}
\end{restatable}

The proof of this theorem is deferred to the Appendix.

%\sw{I used simpler arguments}
% Before we proceed to prove the theorem above, we include lemma in
% \cite{KM02} translates the quality of an approximate Nash equilibria
% in $\hat{\mathcal{G}}$ back to the original game $\mathcal{G}$.
% \begin{lemma}[\cite{KM02}]
% Let $\vec{p}$ be any $\beta$-Nash equilibrium for the
% $\alpha$-approximate summarization game $\hat{\mathcal{G}}$. Then
% $\vec{p}$ is a $(2\rho\alpha + \beta)$-Nash equilibrium for
% $\mathcal{G}$. 
% \end{lemma}

% \begin{lemma}
% Let $\hat{\mathcal{G}}$ be the $\alpha$-approximate game. Let
% $\vec{p}$ be any mixed strategy such that $s = \mathbb{E}_{\vec{x}
%   \sim \vec{p}} S(\vec{x})$. Then $\hat{a}_i(s)$ is a $(\gamma\rho +
% 2\rho\alpha)$-best response for player $i$ to $\vec{p}$ in $\hat{\mathcal{G}}$.
% \end{lemma}





==> Selection.tex <==
\section{Equilibrium Selection}\label{s.select}
% Add details about how this computes the highest welfare approximate
% equilibrium that can be found in this way. If $S$ can take on finitely
% many values (i.e. discrete), we can compute all approximate equilibria
% (simply by setting $\alpha$ so that we try all values), and thus
% select the highest welfare approximate equilibrium of the game. We
% discuss approximation for continuous valued $S$ in Section
% \ref{s.exten}.

The previous section discusses how to compute a approximate Nash
equilibrium privately. However, it does not guarantee the quality of
the equilibrium we obtain. This section we propose an algorithm to
select the approximate Nash equilibrium of the highest quality. 
We have the following assumptions:


% \begin{itemize}
% \item \textbf{Discrete Summarization:} $S(\vec{x}) \in \{1/m,2/m, \ldots ,
%   1\}$ and $m = \poly(n)$\footnote{
% In fact, discrete summarization value is a natural assumption when
% each player has a discrete set of actions. But the assumption that
% there are  $\poly(n)$ possible summarization values is more restricted
% than $2^n$ in the most general setting.
% }
% \item \textbf{Separable Summarization:} $S(\vec{x}) = \sum_{i=1}^n f_i(x_i)$
% \item \textbf{Monotone Quality:} The quality of a strategy profile is
% measured by a quality function $q$ (e.g. social welfare) on a
% summarization value such that $q$ is a monotone increasing (or
% decreasing) function.
% \end{itemize}

\paragraph{Assumption 1}{Each player $i$ has an ordering over the action
  set $\A$: $b_0 \succ b_1$ if and only if $S(b_0, x_{-i}) \geq
  S(b_1, x_{-i})$ for any $x_{-i} \in \A^{n-1}$. We say player $i$ is playing
  \emph{optimistically} if she is maximizing the summarization value
  with her action, and playing \emph{pessimistically} if minimizing. }

\paragraph{Assumption 2}{Let $q\colon [0,1] \rightarrow [0,1]$ be a
  score function that measures the quality of a summarization value. We
  assume that $q$ is $\lambda$-Lipschitz.}
\newline

\sw{Define the benchmark we are competing against. Our algorithm
  allows us to the best $4\rho\gamma$-approx-pure nash. Does exact pure nash
  always exist though? Also, KM'02 gives a constructive proof to
  $3\rho\gamma$-approx pure nash specific to summarization game. In
  general large games, we can derive a weaker bound using Chernoff:
  $O(\gamma \log{n}/\sqrt{n})$, say $\gamma = 1/n$. }

\citet{KM02} shows that there exists an $O(\gamma\rho)$-approximate
pure Nash equilibrium for any $(\rho, \gamma)$-summarization game. Let
$\OPT$ be highest $q(\vec{x})$ for any $\sigma$-approximate Nash
equilibrium $\vec{x}$ of the game for $\sigma = 4\rho\gamma$. We
show that our algorithm can compute an $O(\sigma +
\rho\gamma)$-approximate equilibrium that gets some additive
approximation to $\OPT$.


We first derive a necessary condition for the equilibria in a
summarization game: each player is playing an $\rho\gamma$-apparent
best response.

\begin{lemma}
\label{lem:nash-prop}
Let $x$ be a pure Nash equilibrium of a $(\gamma,
\rho)$-summarization game $\mathcal{G}$, and let $S(x) = s$. Then
for any action $b\in \A$, we must have 
\[
\F_{x_i}^i(s) \geq \F_{b}^i(s) - \rho\gamma. 
\]
\end{lemma}

\begin{proof}
Without loss of generality, suppose $x_i = 1$. Let $s' = S(0,
x_{-i})$. Since $x$ is an Nash equilibrium, we know that $\F^i_1(s)
\geq \F^i_0(s')$. By the bounded influence of player $i$, we know that $|s - s'| \leq \gamma$.
Also, since the utility function of $i$ is $\rho$-Lipschitz, we have
that $|\F^i_0(s') -  \F^i_0(s)| \leq \rho\gamma$. It follows that
$\F^i_0(s') \geq \F^i_0(s) - \rho\gamma$, and therefore $\F^i_1(s)
\geq \F^i_0(s)$.
\end{proof}



\paragraph{Remark}{ For each Nash equilibrium $x$ with summarization
value $s$, it is not necessarily true that $\F_{x_i}^i(s) \geq
\F_b^i(s)$. But we can still guarantee that each player $i$ is
playing $\rho\gamma$-apparent best response. }
\newline

The full algorithm is presented in \Cref{alg:pselection}, and like the
previous algorithm, it iterates through a discretized set of
summarization values $\{0,\alpha,\ldots , 1-\alpha\}$. At each
summarization value $s$, we let each player compute
$\rho\gamma$-apparent best response set
% we try to find
% whether there exists an approximate equilibrium that has approximately
% the same summarization value and output as soon as we obtain one. This
% will guarantee that the quality of our output equilibrium is at least
% as good as the best pure Nash equilibrium.
% \footnote{ This is because
%   we are starting from the largest $s$. Note that the monotone
%   condition is not necessary, as we just need an ordering of the
%   summarization values such that $q(s_1) \geq q(s_2) \ldots \geq
%   q(s_m)$. Yet, $\poly(n)$ summarization values is still a stronger
%   assumption compared to $2^n$ possible values in the most general
%   case. }
$a_i(s)\subseteq \{b\mid \F_{b}^i(s) \geq \F_{1 - b}^i(s) -
\rho\gamma\}$ summarization value $s$, and let $X(s) = \{\vec{x} \mid
\mbox{each player has } x_i\in a_i(s) \}$. Thus, if there is an Nash
equilibrium $x$ with $s = S(x)$, we must have $x \in X(s)$ by
\Cref{lem:nash-prop}. We use this as a guidance to find our
approximate equilibrium: if any strategy profile $x'\in X(s)$
satisfies $|S(x') - s| \leq \beta$, we could argue that $x'$ is an
$O(\rho\gamma + \beta\rho)$-Nash equilibrium.

Note that the cardinality of $X(s)$ can potentially be $\Omega(2^n)$,
but we can simply compute 
\[S_{max} = \max_{x\in X(s)} S(x) \mbox{, and }
S_{min} = \min_{x\in X(s)} S(x)
\] by asking players to play
optimistically and pessimistically. Then there are three cases: either
$S_{max}$ or $S_{min}$ is close to $s$, or $s\in [S_{min}, S_{max}]$.
In the first two cases, we can simply output the two corresponding
optimistic or pessimistic strategy profile. In the last case, we can
perform the same smooth walk as in \Cref{alg:psn} from $x_{max}$ to
$x_{min}$ and output an intermediate profile $x'$ that satisfies
$|S(x') - s| \leq \beta$.

Furthermore, we are also interested in computing the best equilibrium.
Let $s_1\succ s_2 \succ \ldots \succ s_{1/\alpha}$ be an ordering over
the set of summarization values $\{0, \alpha, \ldots, 1-\alpha\}$ such
that $q(s_{i}) \leq q(s_{i+1})$. The algorithm will compute an
approximate equilibrium with summarization value closet to the highest
$s_i$ possible. Let $\OPT(r)$ be the optimal quality value for
all $r$-approximate equilibria, and our goal is to find an $O(r +
\gamma\rho)$-approximate equilibrium with quality score at least
$\OPT(r) - \lambda\alpha$.





\begin{algorithm}[h!]
  \caption{Private Equilibrium Selection}
  \label{alg:pselection}
  \begin{algorithmic}
    \INDSTATE[0]{\textbf{Input}: A discrete $(\gamma,
      \rho)$-summarization game $(S, \{(\F_b^i)\}_{i=1}^n)$,
      and a privacy parameter $\eps$}
    \INDSTATE[0]{\textbf{Output:} An $(\xi + 7\rho\gamma)$-approximate Nash equilibrium with
    the  quality score at least $\OPT(4\rho\gamma) - \xi\lambda/10\rho$}
  \INDSTATE[1]{\textbf{let} $\alpha = \xi / 10\rho$}
  \INDSTATE[1]{\textbf{For} each summarization value $s\in \{0,
    \alpha, \ldots, 1-\alpha\}$} \INDSTATE[2]{\textbf{For} each player
    $i$ \textbf{let} $a_i(s)\subseteq \A$ be the $(2\alpha\rho + 5\rho\gamma)$-apparent
    best response set.} \INDSTATE[2]{\textbf{let} $X(s) = \{\vec{x}
    \mid \mbox{each player has } x_i\in a_i(s) \}$}
  \INDSTATE[2]{\textbf{let} $S_{max}(s) = \max_{x\in X(s)} S(\vec{x})$
    and $S_{min}(s) = \min_{x\in X(s)} S(\vec{x})$}
  \INDSTATE[1]{\textbf{let} $\{s_1, s_2 \ldots, s_n\}$ be an ordering
    of $\{0, \alpha, \ldots , 1-\alpha\}$ such that $q(s_i) \geq
    q(s_{i+1})$ for each $s_i$}


  \INDSTATE[1]{\textbf{For} $1\leq k \leq 1/\alpha$, \textbf{let} queries}
  \[
  Q_k = |S_{max}(s_k) - s_k| \qquad Q_k' = |S_{min}(s_k) - s_k|
  \]
  \[
  Q_k'' = \max\left(\min\left( S_{min}(s_k) - s_k, 0 \right),
    - 2\alpha \right) + \max\left(\min\left( s_k - S_{max}(s_k), 0 \right),
    - 2\alpha \right)
  \]
  \INDSTATE[1]{\textbf{let} $\{a_k\} = \SV(\{\F_b^i\}, \{Q_k\},
    3\alpha, 1, \eps/4)$}
  \INDSTATE[2]{\textbf{if} some $a_i\neq \perp$ \textbf{then Output} $x_{max}(s_i)$}
  \INDSTATE[1]{\textbf{let} $\{a'_k\} = \SV(\{\F_b^i\}, \{Q'_k\},
    3\alpha, 1, \eps/4)$}
  \INDSTATE[2]{\textbf{if} some $a'_i\neq \perp$ \textbf{then Output} $x_{min}(s_i)$}

 % \INDSTATE[3]{Use
 %    $\SV$ to determine whether $|S_{max} -s| \leq \alpha$ or $|S_{min}
 %    - s| \leq \alpha$ or $S_{min} < s < S_{max}$ }

  \INDSTATE[1]{\textbf{let} $\{a''_k\} = \SV(\{\F_b^i\}, \{Q''_k\},
    3\alpha, 1, \eps/4)$} \INDSTATE[2]{\textbf{if} some $a''_l \neq
    \perp$ \textbf{then } }
    \INDSTATE[2]{\textbf{for} each $0\leq j\leq n$, \textbf{let}
      strategy profile $x^j$ be defined as}
    \[
    x^j_i = \begin{cases}
      x_{max}(s_l)_i \mbox{ if }i\leq j\\
      x_{min}(s_l)_i \mbox{ otherwise}
      \end{cases}
    \]
      \INDSTATE[3]{\textbf{let } query $Q_j''' = S(x^j)$} 
    \INDSTATE[3]{\textbf{let} $\{a'''_j\}=\SV(\{\F_b^i\}, \{Q_j'''\},
      \gamma/2 + \alpha, 1, \eps/4)$}
    \INDSTATE[4]{\textbf{if} some $a'''_{j'} \neq \perp$  \textbf{then
        Output } $x^{j'}$ \textbf{else } Abort.} 
    \INDSTATE[1]{\textbf{else} Abort.}

\end{algorithmic}
\end{algorithm}

\begin{theorem}
\Cref{alg:pselection} satisfies $\eps$-joint differential privacy.
\end{theorem}

\begin{proof}
Basically the same proof as \Cref{thm:psn-privacy}.
\end{proof}


\begin{restatable}{theorem}{pselection}
\label{thm:pselection}
Suppose $\gamma = 1/n$, then with probability at least $1 - \beta$,
\Cref{alg:pselection} outputs an $(\xi + 7\rho\alpha)$-approximate
Nash equilibrium that quality score at least $\OPT(4\rho\gamma) -
\xi\lambda/10\rho$, as long as $n\geq \tilde{O}(\rho\log(1/\beta)/\xi\eps)$.
\end{restatable}




%\subsection{Selection Based on More General Function}

%\sw{This section should subsume the previous result, since we allow
%  the welfare/quality function to be a function of the strategy profile.}

%\paragraph{Assumption}{Let $SW\colon \A^n \rightarrow [0,1]$ be a
%  welfare function that measures the quality of a state in the game.
%  We assume that $SW$ is $\lambda$-Lipschitz.}

%\sw{Stuck here...}










==> parti.tex <==
\section{Application: participation in private computation}


\subsection{Private Computation}
One application of this algorithm is to the setting studied by
\cite{GL13}, where a data analyst wishes to publish a statistic using
the private data of individuals, but first must convince individuals
to share their data\footnote{This is often called the ``Sensitive
Surveyor's problem,'' see \cite{Rot12}}. These individuals may
experience some loss from having their data used in the computation,
but experience some utility from having the computation
performed\footnote{Maybe the output is useful to the individual, such
as personalized recommendation, or maybe the individual is a good
Samaritan, who is willing to share her data as long as it's not
\emph{too} revealing}. Much of the differential privacy literature
assumes that the analyst can promise $\epsilon$-differential privacy
to each user, for some fixed $\epsilon$. In practice, these types of
guarantees are typically not offered. More likely, the analyst may
announce how this data will be used, and (if we're lucky) a particular
computation that will be performed on the data acquired.

Motivated by this fact, \cite{GL13} consider a setting where the analyst announces a computation to be
performed and a fixed level of noise that will be added to the output.
Agents can then decide whether or not to participate in this
computation, and the actions $0$ and $1$ correspond respectively to
opting out or opting into the computation. Since the level of noise is
fixed, then the privacy guarantee to each agent depends on the total
number of individuals who opt in to the computation. For example, when
the analyst adds noise $Lap(1/\epsilon)$ to a computation with
sensitivity $1/n$, this preserves $\epsilon/n$-differential privacy
for each participating agent.

\cite{GL13} looked at Bayes-Nash equilibrium of this large game. Such an equilibrium concept requires
each agent to have a Bayesian prior over the utilities and privacy
costs of the rest of the population. For large games, it may be
impractical to assume that each individual is so informed about all
other players. Our approach searches instead for an (approximate) ex
post Nash equilibrium of this game, which doesn't require individuals
to have any information about the types or privacy costs of the
population.

They also highlight the multiplicity of Bayes-Nash equilibria and the
existence of ``bad'' (low participation) equilibria in this game. They show that as
the level of announced noise increases, while every existing
equilibrium improves\footnote{Here ``better'' corresponds to higher
participation, and ``worse'' corresponds to lower participation}, new
equilibria may arise that are have lower participation than the
previous ``worst'' equilibrium. Running our PrivateEquilibriumSelection algorithm avoids this issue because
it allows for the designer to select the equilibrium with the highest
participation for a given level of noise. Note that this allows the
designer to find an (approximate) equilibrium that simultaneously
maximizes welfare of the individuals and maximizes participation the
competition (thus reducing sampling error). 

\subsection{Instantiation of a (Monotone) Aggregative Game}
Now this model can be seen as an instantiation of the aggregator
game. The players have binary actions: opt-in and opt-out,
corresponding to 1 and 0. The aggregator function is the proportion
of the population that participate $S(\vec{x}) = 1/n \sum_{i=1}^n
x_i$. The influence of each player on $S$ is bounded by $1/n$. In
addition, we assume the  utility functions of the agents are
$\rho$-Lipschitz. Furthermore, if agent $i$ has private threshold
$T\in [0,1]$, then we can interpret this as $\F^i_1(t) < \F^i_0(t)$ 
for $t < T$, and $\F^i_1(t) \geq \F^i_0(t)$ for $t \geq T$.

Notice that the function $V$ in this setting satisfies the monotone
increasing property: $V(s_1) \geq V(s_2)$ for any $s_1 > s_2$.
Intuitively, if an agent is told that more people have opted-in,
she would be more willing to participate, so at least as many people
would decide to opt-in. We say a aggregative game is \emph{monotone}
if the function $V$ satisfies such a monotone property.


\begin{lemma}
Let $\mathcal{G}$ be a monotone $(\rho, \gamma)$-aggregative game.
Then \Cref{alg:psn} finds an approximate Nash equilibrium in Case 1. 
\end{lemma}

\begin{proof}
We show that if $V$ satisfies the monotone property, we must have
$V(k\alpha) \in I_k$ for some index $k$. 

Suppose not. Then we know that $V(0) > \alpha$ and $V(1 - \alpha) < 1
- \alpha$. It follows that there exists $m$ such that 
\[
V(I_m)   \geq \alpha  (m + 1) \mbox{ and }
V(I_{m+1}) < \alpha  (m + 1)
\]
, which implies that $V(I_m) > V(I_{m+1})$, a contradiction to monotonicity. 
\end{proof}

Therefore, we can compute an approximate Nash equilibrium for the
private computation in Case 1 of the \Cref{alg:psn}. 






%\subsection{Maximizing total accuracy of computation}\label{s.maxacc}

%We now look at selecting the optimal noise level to maximize accuracy by managing the trade-off between adding noise and sampling error from individuals who opted out.

%When privacy costs are correlated with private data, then the non-participating agents may induce a bias in the data we observe, which can greatly decrease the accuracy.  In this case, there are two possible sources of error that may reduce accuracy: (1) non-participating agents, and (2) noise added for privacy.  Both of these error sources are affected by the choice of $\epsilon$: as $\epsilon$ increases, more agents will choose to participate (in the best equilibrium), but more noise needs to be added.  We can easily get a 2-approximation to the best accuracy by choosing $\epsilon$ such that the error from these two sources are equal.
%\[2 \cdot max\{ \text{non-participation error}, \text{noise error} \} \; \leq \text{non-participation error} + \text{noise error} \]
%Can we do better?  This may be related to what Katrina and Juba are thinking about.

%\subsection{Local privacy}

%In the local privacy model, the agents do not trust the mediator and
%they report their best response via a $\eps$-local randomizer defined
%as follows:

%\begin{definition}[Local Randomizer]
%An $\eps$-local randomizer $R\colon \cX \rightarrow
%R$ is an $\eps$-differentially private algorithm that takes a database
%of size 1.
%\end{definition}

%\begin{definition}[Local Algorithm]
%An algorithm is $\eps$-local if it accesses the database $D$ via the
%oracle $LR_D$ with the following restriction: If $LR_D(i, R_1),\ldots
%, LR_D(i, R_k)$ are the algorithm's invocations of $LR_D$ on index $i$,
%where each $R_J$ is an $\eps_j$-local randomizer, then $\eps_1 +
%\ldots + \eps_k\leq \eps$. 
%\end{definition}

%The role of the mediator is to survey the best responses from all
%agents given the aggregator value is some $k\alpha$. To satisfy
%$\eps$-local privacy, each agent answers truthfully with probability
%$p = 2e^\eps/(e^\eps +1)$ and submit the opposite response with
%probability $1 - p$. Alternatively, an instantiation of a local
%private mechanism would simply be the agents adding noise sampled from
%$\Lap(1/\eps)$ to their responses. The following lemma helps us to
%bound the sum of a collection of Laplace random variables. 

%\begin{lemma}[\citet{chan-counter}]
%Let $Z_1, \ldots, Z_n$ be independent random variables sampled from
%$\Lap(b)$.  Suppose $Y = \sum_i Z_i$ and $0 < \lambda < 2\sqrt{2}nb$.
%Then \[
%\Pr[Y > \lambda] \leq \exp\left( - \frac{\lambda^2}{8nb^2} \right).
%\]
%\end{lemma}
% \sw{TODO: use Chernoff bound to get an error bound here.}
% With probability $p$ they answer truthfully, and with probability
% $1-p$ they submit a random response to the query. This introduces an
% additional $\sqrt{n}$ error to each query response. Using sparse
% vector analysis, we calculate the first intersection of the function
% $v(S)$ with the diagonal and still only accumulate error from a single
% query.  If such an intersection exists, then we know we have found an approximate
% equilibrium. Note that the approximate equilibrium can still be
% computed, but the approximation factor is worse than in the standard
% differential privacy setting.

%This means with probability at least $1 - \beta$, the error computing
%a aggregator function with $\eps$-local privacy is bounded by
%$O\left(\frac{\log(1/\beta)}{\sqrt{n} \eps} \right)$. In other words,
%we can compute $m$ different aggregator values as long as $m$ is
%much smaller than $\sqrt{n}$.

%Note that $\Cref{alg:psn}$ requires asking
%$O(n)$ queries, as in Case 2 we flip bits walking from the strategy profile at
%$V(k\alpha)$ to the strategy profile at $V((k+1)\alpha)$. We don't
%know how to handle this case in the local privacy model because it
%requires $n$ queries. % From above, we see that we can only privately answer $\sqrt{n}$ queries privately with non-trivial accuracy, so we cannot compute an approximate equilibrium in this setting.

%However, if the best response aggregator function $V(S)$ is monotone, then
%we are guaranteed the algorithm runs in Case 1, where $V(S)$ intersects
%the diagonal. This shows that our result extends to the local privacy
%model, as long as $V(S)$ is monotone.
 % Monotonicity of $V(S)$ is
% implied by a single crossing condition on the agents' utilities for
% each action, $\F^i_0$ and $\F^i_1$.
% Under this condition, the agent's
% best response function can be described using a single threshold
% $r_i$, where for $S \in [0,r_i)$, agent $i$'s best response is action
% 0, and for $S \in [r_1, 1]$, agent $i$'s best response is action 1.

% \rc{Rest of section is about ensuring IR when data is correlated with
% privacy costs (e.g. this may be why we use local privacy). I don't
% know if we'll want to keep this.}
% \sw{Commented out for now.} 

% Another
% concern that arises in the local privacy model, is that agents may
% experience a loss, simply by responding to the designer's query that
% computes $v(S)$. This is particularly true when privacy costs are
% themselves private as a result of correlations between data and
% privacy costs. Such a effect can violate individual rationality if the
% utility an agent enjoys from the outcome of the mechanism is not
% sufficient to compensate her privacy loss from responding to the
% query.

% One approach to address this was used in \cite{NOS12} is to only
% guarantee individual rationality for agents with privacy costs that
% were ``not too large,'' namely below some upper bound $c_{max}$.
% (Think of $c_i$ as the cost of agent $i$ for sharing her data with the
% mechanism designer.) They provide a technical condition under which
% the upper bound $c_{max}$ grows with $n$, and the fraction of agents
% who experience costs $c_i > c_{max}$ diminishes as $n$ gets large.

% They consider a similar model where participating gives some positive
% utility $u$, and non-participation gives utility $0$. Agents also
% experience a privacy loss from participating in an
% $\eps$-differentially private computation, and this loss is upper
% bounded by $c_i \cdot \eps$. As in \cite{GL13}, individual rationality
% gives that agents will participate in the game if their gain from
% participation minus their privacy loss is greater than zero. By
% setting $c_{max} = O(n^{\alpha})$ and $\epsilon(n) = n^{-\alpha}$, we
% can ensure that the upper bound on privacy loss ($c_{max} \cdot
% \epsilon$) goes to zero as $n$ get large, for all players with privacy
% costs smaller than $c_{max}$.

% To ensure that only a diminishly small fraction of the agents have
% privacy costs above $c_{max}$, they introduce a technical condition on
% the distribution of values, called $(\alpha, \beta)$-admissibility.
% They say that a distribution $\mathcal{D}$ is $(\alpha,
% \beta)$-admissible if
% \[Pr_{c\sim \mathcal{D}} [c> n^{\alpha}] = O(n^{-\beta}) \] They
% remark that the Normal distribution satisfies (a stronger version of)
% this condition, and all distributions that have a finite $p^{th}$
% moment are $(\alpha, \beta)$-admissible for all $\beta \leq p \alpha$.

% One drawback to using this is that is requires a distribution on
% privacy valuations, which is what we were trying to avoid. Perhaps
% it's not too much to ask that the designer knows the distribution of
% types, but the agents don't need to know it? Another issue is that
% this construction requires us to set $\epsilon$ as a function of $n$,
% which may conflict with selecting the optimal $\epsilon$ to maximize
% accuracy, as in Section \ref{s.maxacc}.


